SpaDE: Improving Sparse Representations using a Dual Document Encoder for First-stage Retrieval

Sparse document representations have been widely used to retrieve relevant documents via exact lexical matching. Owing to the pre-computed inverted index, it supports fast ad-hoc search but incurs the vocabulary mismatch problem. Although recent neural ranking models using pre-trained language models can address this problem, they usually require expensive query inference costs, implying the trade-off between effectiveness and efficiency. Tackling the trade-off, we propose a novel uni-encoder ranking model, Sparse retriever using a Dual document Encoder (SpaDE), learning document representation via the dual encoder. Each encoder plays a central role in (i) adjusting the importance of terms to improve lexical matching and (ii) expanding additional terms to support semantic matching. Furthermore, our co-training strategy trains the dual encoder effectively and avoids unnecessary intervention in training each other. Experimental results on several benchmarks show that SpaDE outperforms existing uni-encoder ranking models.

==> Tables/tab_dataset.tex <==
\begin{table}[]
\caption{Detailed statistics on test dataset for MS MARCO passage corpus. Note that average number of tokens per query is based on WordPiece tokenizer.}
\label{tab:dataset}
\centering
\begin{tabular}{c|cccc}
\toprule
Dataset              & \#queries & \#judges/\textit{q} & \#rel/\textit{q} & \#tokens/\textit{q} \\ \midrule
MS MARCO dev.          & 6,980       & 1.1            & 1.1                    & 7.02        \\
TREC DL 2019              & 43         & 215.3           & 58.2                    & 7.02         \\
TREC DL 2020              & 54         & 210.9           & 30.9                    & 7.22        \\ \bottomrule
\end{tabular}
\end{table}
